DeTriever: Decoder-representation-based Retriever for Improving NL2SQL In-Context Learning

While in-context Learning (ICL) has proven to be an effective technique to improve the performance of Large Language Models (LLMs) in a variety of complex tasks, notably in translating natural language questions into Structured Query Language (NL2SQL), the question of how to select the most beneficial demonstration examples remains an open research problem. While prior works often adapted off-the-shelf encoders to retrieve examples dynamically, an inherent discrepancy exists in the representational capacities between the external retrievers and the LLMs. Further, optimizing the selection of examples is a non-trivial task, since there are no straightforward methods to assess the relative benefits of examples without performing pairwise inference. To address these shortcomings, we propose DeTriever, a novel demonstration retrieval framework that learns a weighted combination of LLM hidden states, where rich semantic information is encoded. To train the model, we propose a proxy score that estimates the relative benefits of examples based on the similarities between output queries. Experiments on two popular NL2SQL benchmarks demonstrate that our method significantly outperforms the state-of-the-art baselines on one-shot NL2SQL tasks.

==> fig/batchsize.tex <==
% \begin{figure*}[tb] %插入图片
% \subfigure[Execution accuracy for different classes on Spider development set.]{
% \begin{minipage}[t]{0.45\columnwidth}{
% %\small
%     \begin{tabular}{ccccc}
%     \toprule
%          Batch size& Easy & Medium & Hard & Extra  \\
%     \midrule
%        16  &  87.5& 66.14& 62.07& 43.37\\
%        32  & 88.71& 67.49& 61.49& 42.77\\
%        48  & 89.03 &68.76&62.57&42.16\\
%        64  & 89.52&69.28&63.79&39.16\\
%     \bottomrule
%     \end{tabular}
% }
% \end{minipage}
% }
% \subfigure[Overall execution accuracy] { 
% \centering %图片居中

% \includegraphics[scale=0.2]{fig/figure_batchsize.pdf}
% % \resizebox{0.33\columnwidth}{!}{
% % \begin{tikzpicture}
% % \begin{axis}[
% % %sharp plot,
% % legend pos=north west,
% % %xmajorgrids=true,
% % xmode=normal,
% % xlabel=Number of batch size, %x坐标名
% % ylabel=Execution Accuracy, %y坐标名
% % ymin=66,
% % ymax=69,
% % %ybar=1pt,% configures `bar shift'
% % %bar width=8pt, 
% % %xmode=log, log ticks with fixed point,
% % enlargelimits=0.1,
% % width=8cm, height=6cm,
% % %x tick label style={shift={(axis cs:0.5,0)},anchor=east,rotate=60,},
% % xtick={16,32,48,64},
% % ]
% %     \addplot+[very thick,mark=square,mark options={scale=0.6}, color=color1] plot coordinates {
% %     (16, 67.12)
% %     (32, 67.6)
% %     (48, 68.11)
% %     (64, 68.38)
% %     %(128,66.73)
% %     };
% %     %\addlegendentry{Overall}
% % \end{axis}
% % \eat{
% % \begin{axis}[
% % %sharp plot,
% % axis y line*=right,%y轴居右
% % axis x line=none,%不画x， 避免线重画
% % legend pos=north west,
% % %xmajorgrids=true,
% % %xmode=normal,
% % %xlabel=Number of batch size, %x坐标名
% % ylabel=Execution Accuracy, %y坐标名
% % ymin=30,
% % ymax=95,
% % ybar=1pt,% configures `bar shift'
% % bar width=8pt, 
% % %xmode=log, log ticks with fixed point,
% % enlargelimits=0.1,
% % width=10cm, height=5cm,
% % %x tick label style={shift={(axis cs:0.5,0)},anchor=east,rotate=60,},
% % xtick={16,32,48,64},
% % ]
% %     \addplot+[ybar,fill=color1,draw=black] coordinates {
% %     (16,87.5)
% %     (32,88.71)
% %     (48, 89.01)
% %     (64, 89.52)
% %     };
% %     %\addlegendentry{Easy}
% %     \addplot+[ybar,fill=color2,draw=black] coordinates {
% %     (16,66.14)
% %     (32,67.49)
% %     (48, 68.11)
% %     (64, 69.28)
% %     };
% %     %\addlegendentry{Medium}
% %     \addplot+[ybar,fill=color3,draw=black] coordinates {
% %     (16,62.07)
% %     (32,61.49)
% %     (48, 62.32)
% %     (64, 63.79)
% %     };
% %     \addplot+[ybar,fill=brown!80!white,draw=black] coordinates {
% %     (16,43.37)
% %     (32,42.77)
% %     (48, 42.32)
% %     (64, 40.16)
% %     };
% %     %\addlegendentry{Hard}
% %     %\addlegendentry{EOS}
% % \end{axis}
% % }
% % \end{tikzpicture}
% % }
% }


% \caption{One-shot ICL results (execution accuracy on development set of Spider dataset) of CodeLlama-13b where the prompt is retrieved by our trained retriever with a different batch size. The one-shot Prompt is retrieved by the one with the largest cosine similarity.} % 设置caption
% \label{fig:batchsize}  % 设置用于reference的label
% \end{figure*}

% \begin{figure}
% \includegraphics{fig/figure_batchsize.pdf}
% \caption{One-shot ICL execution accuracy on Spider where \ourmethod is trained with different batch sizes.
% \label{fig:batchsize}
% \end{figure}

\begin{figure}
\begin{floatrow}
\ffigbox{%

}
{%
  \caption{One-shot ICL execution accuracy on Spider where \ourmethod is trained with different batch sizes.
  % (execution accuracy on development set of Spider dataset) of CodeLlama-13b where the prompt is retrieved by our trained \ourmethod~with a different batch size. The one-shot prompt is retrieved by the one with the largest cosine similarity.
  }%
  \label{fig:batchsize}
}
\capbtabbox{%
  \begin{tabular}{ccccc}
    \toprule
         Batch size& Easy & Medium & Hard & Extra  \\
    \midrule
       16  &  87.5& 66.14& 62.07& 43.37\\
       32  & 88.71& 67.49& 61.49& 42.77\\
       48  & 89.03 &68.76&62.57&42.16\\
       64  & 89.52&69.28&63.79&39.16\\
    \bottomrule
    \end{tabular}
}{%
  \caption{One-shot ICL execution accuracy for different classes on Spider development set of \ourmethod.}%
  \label{tab:diffresult}
}
\end{floatrow}
\end{figure}
